Scheduling and control over networks using MPC with time-varying terminal ingredients: extended version

Rollout approaches are an effective tool to address the problem of co-designing the transmission schedule and the corresponding input values, when the controller is connected to the plant via a resource-constrained communication network. These approaches typically employ an MPC, activated at multiples of the period length of a base transmission schedule. Using multi-step invariant terminal regions and a prediction horizon longer than the base period, stability can be ensured. This strategy, however, suffers from intrinsic shortcomings, such as a high computational complexity and low robustness. We aim to resolve these drawbacks by proposing an MPC with periodically time-varying terminal region and cost for the rollout setup, where the controller is activated at each time instant and features an arbitrary but fixed prediction horizon. We consider in more detail two specific setups from the literature on Networked Control Systems, namely the token bucket network and actuator scheduling. For both setups, we provide conditions for which convergence under application of the time-varying MPC can be guaranteed. In two numerical examples, we demonstrate the benefits of the proposed method.

==> customCommands.tex <==
% symbol to end Theorems, Definitions, Remarks, ...
\newcommand{\oprocendsymbol}{{$\bullet$}} 					% symbol to end Theorem/Lemmata/...
% \newcommand{\oprocend}{\relax\ifmmode\else\unskip\hfill\fi\oprocendsymbol}
\def\oprocend {{%        set up
\parfillskip=0pt        % so \par doesnt push \square to left
\widowpenalty=10000     % so we dont break the page before \square
\displaywidowpenalty=10000  % ditto
\finalhyphendemerits=0  % TeXbook exercise 14.32
%
%                 horizontal
\leavevmode             % \nobreak means lines not pages
\unskip                 % remove previous space or glue
\nobreak                % don’t break lines
\hfil                   % ragged right if we spill over
\penalty50              % discouragement to do so
\hskip.45em              % ensure some space
\null                   % anchor following \hfill
\hfill                  % push \square to right
\oprocendsymbol%              % the end-of-proof mark
%
%                   vertical
\par}}                  % build paragraph










==> myStandardPreamble_arXiv.tex <==
% change @-symbol interpretation for using macros
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% =============================
% ===         M I S C      ====
% =============================

% extended TeX
\@ifpackageloaded{etex}{}{\RequirePackage{etex}}

% keeps relative paths when including different .tex-files
% use \subimport*{subdirectory}{tex-File} to input tex-Files
\@ifpackageloaded{import}{}{\usepackage{import}}

% nice tables
\@ifpackageloaded{booktabs}{}{\usepackage{booktabs}}

% microtype for better spacing of letters
%\@ifpackageloaded{microtype}{}{\usepackage{microtype}}

% calculations also in tex-Code
\@ifpackageloaded{calc}{}{\usepackage{calc}}

% if conditions
\@ifpackageloaded{ifthen}{}{\usepackage{ifthen}}



% =============================
% ===    G R A P H I C S    ===
% =============================
\@ifpackageloaded{graphicx}{}{\usepackage{graphicx}}
\@ifpackageloaded{xcolor}{}{\usepackage{xcolor}}


% =============================
% ===         T I K Z      ====
% =============================
\@ifpackageloaded{tikz}{
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
     }{
     \usepackage{tikz}
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
}
\@ifpackageloaded{pgfplots}{
     }{
     \usepackage{pgfplots}
     }
% SOME TIKZ STYLE DEFINITIONS
\tikzstyle{boxstyle}=[draw=black,inner sep=7pt]      % style for boxes in blockdiagrams
\tikzstyle{arrowstyle}=[]                            % style for arrows in blockdiagrams



% =============================
% ===         M A T H      ====
% =============================
\@ifpackageloaded{amsmath}{}{\usepackage{amsmath}}
\@ifpackageloaded{amsfonts}{}{\usepackage{amsfonts}}
\@ifpackageloaded{amssymb}{}{\usepackage{amssymb}}
\let\theoremstyle\relax
\@ifpackageloaded{amsthm}{}{\usepackage{amsthm}}
\@ifpackageloaded{yhmath}{}{\usepackage{yhmath}}
\@ifpackageloaded{mathdots}{}{\usepackage{mathdots}}


% =============================
% ===    H Y P E R R E F    ===
% =============================

% some color definitions
\colorlet{lcolor}{green!45!black}
\colorlet{ucolor}{magenta!40!black}
\colorlet{ccolor}{green!40!black}

% hyperref for internal links
\usepackage[colorlinks=true,%
            linkcolor=lcolor,%
            urlcolor=lcolor,%
            citecolor=lcolor]{hyperref}

% cleverref for automatically labeling of references
\usepackage[nameinlink]{cleveref}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% rechange @-symbol interpretation
\makeatother

